PerceptTwin: Semantic Scene Reconstruction for Iterative LLM Planning and Verification

Simulation environments are useful for both robot policy learning and planning verification and validation. Traditionally, the process of creating a simulation was onerous. Creating a bespoke simulation environment for each individual environment that a robot would operate in was simply infeasible. In this work, we introduce PerceptTwin, a fully automatic pipeline that constructs interactive simulations directly from semantic scene representations produced by a robot's perception stack. PerceptTwin combines open-vocabulary object maps with 3D asset generation, affordance prediction, and commonsense condition checking. These interactive simulations can be used to validate and refine plans before they are executed on the robot hardware. Borrowing from the AI alignment literature, we also introduce an LLM judge that verifies plan correctness and alignment with human preferences. Experiments show that PerceptTwin feedback allows LLM planners to refine plans, enhance safety, and resist harmful black-box prompting attacks. In our suite of tasks, PerceptTwin improves plan success by an average of approximately 39% for GPT5, GPT5Mini, and GPT5Nano planners. Additionally, PerceptTwin also improves human plan verification by up to 18% on average for plans that fail due to unfilled skill preconditions. Our results demonstrate the potential of open-vocabulary scene simulation from robot perception as a foundation for safer, more reliable robot planning.

==> chatbox/chats.tex <==
\ProvidesFile{chats.tex}[2025/09/04 Chatbox environments - fixed]
\RequirePackage[most]{tcolorbox}
\RequirePackage{graphicx}
\RequirePackage{fancyvrb}
\RequirePackage{xcolor}
\RequirePackage{tikz}

% Counter for sessions
\newcounter{chatcounter}
\setcounter{chatcounter}{1}


% Chat session box
\newtcolorbox{chatsession}[2][]{%
  enhanced,
  sharp corners,
  colback=white,
  colframe=blue!40,
  fonttitle=\bfseries, 
  title=\hspace{1em}Chat~\thechatcounter\refstepcounter{chatcounter}:~#1,
  left=3mm,
  %top=1mm, bottom=1mm,
  %#1
  overlay={
      \node[anchor=north west, xshift=0pt, yshift=0pt] at (frame.north west)
        {\includegraphics[height=1em]{chatbox/icons/chat.png}};
    }
}



\tcbset{
  chatbox/.style={
    enhanced,
    sharp corners=south,
    boxrule=0.8pt,
    colback=gray!5,
    colframe=blue!40,
    drop shadow={black!30!white},
    fonttitle=\bfseries,
    left=3mm,
    %before upper={\includegraphics[height=1em]{#1}\hspace{2mm}},
    %top=1mm, bottom=1mm,
    overlay={
      \node[anchor=north west, xshift=0pt, yshift=1pt] at (frame.north west)
        {\includegraphics[height=1em]{#1}};
    },
  }
}

\newtcolorbox{humanchat}{
  chatbox={chatbox/icons/human.png},
  title=\hspace{1em}Human
}

\newtcolorbox{attackerchat}{
  chatbox={chatbox/icons/human.png},
  title=\hspace{1em}Attacker
}

\newtcolorbox{robotchat}{
  chatbox={chatbox/icons/robot.png},
  title=\hspace{1em}Robot
}

\newtcolorbox{scriptchat}{
  chatbox={chatbox/icons/script.png},
  title=\hspace{1em}Software
}

\newtcolorbox{simulationchat}{
  chatbox={chatbox/icons/script.png},
  title=\hspace{1em}Simulation
}

\newtcolorbox{judgechat}{
  chatbox={chatbox/icons/judge.png},
  title=\hspace{1em}Judge
}

\newtcolorbox{llmchat}{
  chatbox={chatbox/icons/llm.png},
  title=\hspace{1em}LLM
}
